Differentially Private Bayesian Persuasion

The tension between persuasion and privacy preservation is common in real-world settings. Online platforms should protect the privacy of web users whose data they collect, even as they seek to disclose information about these data to selling advertising spaces. Similarly, hospitals may share patient data to attract research investments with the obligation to preserve patients' privacy. To deal with these issues, we develop a framework to study Bayesian persuasion under differential privacy constraints, where the sender must design an optimal signaling scheme for persuasion while guaranteeing the privacy of each agent's private information in the database. To understand how privacy constraints affect information disclosure, we explore two perspectives within Bayesian persuasion: one views the mechanism as releasing a posterior about the private data, while the other views it as sending an action recommendation. The posterior-based formulation helps consider privacy-utility tradeoffs, quantifying how the tightness of privacy constraints impacts the sender's optimal utility. For any instance in a common utility function family and a wide range of privacy levels, a significant constant utility gap can be found between any two of the three conditions: $\epsilon$-differential privacy constraint, relaxation $(\epsilon,\delta)$-differential privacy constraint, and no privacy constraint. We further geometrically characterize optimal signaling schemes under different types of constraints ($\epsilon$-differential privacy, $(\epsilon,\delta)$-differential privacy and Renyi differential privacy), all of which can be seen as finding concave hulls in constrained posterior regions. Meanwhile, by taking the action-based view of persuasion, we provide polynomial-time algorithms for computing optimal differentially private signaling schemes, as long as a mild homogeneous condition is met.

==> archive/computational_results_simple.tex <==
\subsection{Homogeneous Agents}
We first consider the case of a single receiver setting and obtain a reduction result, which can also be used in multiple receivers' setting. We additionally assume that action space is finite.  
Since \Cref{num-signal-action} holds, using the same number of signals as actions suffice.
We then abuse the notation $a$ to denote the corresponding signal. Program \eqref{program-distribution} can be written as\footnote{For partial privacy, we substitute $\adjacent_\pset$ for $\adjacent$.}
\begin{align}\label{program-distribution2}
&\max_{\pi} \quad \sum_{\theta\in\Theta}\sum_{a} \pi(a|\theta)\mu(\theta)v(a,\theta)\notag\\
& \begin{array}{r@{\quad}l@{}l@{\quad}l}
s.t.& \sum_{\theta} u(a,\theta)\pi(a|\theta)\mu(\theta)\geq \sum_{\theta} u(a^\prime,\theta)\pi(a|\theta)\mu(\theta), & \text{ for all }a,a^\prime\\
&\sum_{a}\max\{0,\pi(a| \theta)-e^\epsilon \pi(a|\theta^\prime)\}\leq \delta, & \text{ for all }(\theta,\theta^\prime)\in\adjacent\\
&\sum_a \pi(a|\theta)=1, & \text{ for all }\theta\\
&\pi(a|\theta)\geq 0, & \text{ for all }a,\theta
\end{array} .
\end{align}

Note that the number of adjacent pairs in $\adjacent$ is exponentially large in most cases, which makes it hard to solve the program in polynomial time.


When considering web users' data in advertising cases, users are often seen as homogeneous, both in terms of prior and utility functions. This means the sender and receiver only care about the aggregate statistics of the database rather than individual users' data.

Let $\phi:\Theta\rightarrow\Omega$ be the projection that only considers the number of 1s in a given state\footnote{For partial privacy, the projection needs to consider the number of 1s among the sensitive bits under privacy protection and non-sensitive bits separately. Mathematically, $\phi_\pset(\theta)\coloneqq (\sum_{i\in \pset}\theta_i,\sum_{i\notin \pset}\theta_i)$.}. That is, $\phi$:
\[
\phi(\theta)\coloneqq \sum_i \theta_i.
\]
% \[
% \phi_\pset(\theta)\coloneqq (\sum_{i\in \pset}\theta_i,\sum_{i\notin \pset}\theta_i).
% \]


  
We then make two assumptions.
\begin{assumption}\label{prior-assump}
    If $\phi(\theta)=\phi(\theta^\prime)$, then $\mu(\theta)=\mu(\theta^\prime)$.
\end{assumption}
\begin{assumption}\label{utility-assump}
    If $\phi(\theta)=\phi(\theta^\prime)$, then $u(a,\theta)=v(a,\theta^\prime)$ and $v(a,\theta)=v(a,\theta^\prime)$ for any $a$.
\end{assumption}

% We use the signal distribution $\pi(s|\theta)$ to write the program here:
% \begin{align*}
% &\max_{\pi} \quad \sum_{\theta\in\Theta}\sum_{s} \pi(s|\theta)\mu(\theta)v(a_s,\theta) \\
% & \begin{array}{r@{\quad}l@{}l@{\quad}l}
% s.t.& \sum_{\theta} u(a_s,\theta)\pi(s|\theta)\mu(\theta)\geq \sum_{\theta} u(a^\prime,\theta)\pi(s|\theta)\mu(\theta), & \text{ for all }s,a^\prime\\
% &\sum_s \pi(s|\theta)=1, & \text{ for all }\theta\\
% &\pi(s|\theta)\geq 0, & \text{ for all }\theta, s
% \end{array} .
% \end{align*}


It is natural to consider the oblivious method \cite{10.1145/3490486.3538302}, where the signal distributions are identical for any states $\theta$ and $\theta^\prime$ such that $\phi(\theta) = \phi(\theta^\prime)$. That is, the signal distribution depends only on the projection $\omega=\phi(\theta)$. 
We can then redefine adjacency under this oblivious scheme. Say $\omega,\omega^\prime$ adjacent if and only if $|\omega-\omega^\prime|=1$. Let $\adjacent^O$ denote the set of all adjacent pairs $(\omega,\omega^\prime)$ here\footnote{For partial privacy, say $\omega=(a,b),\omega^\prime=(a^\prime,b^\prime)$ adjacent if $|a-a^\prime|=1$ and $b=b^\prime$. Let $\adjacent_\pset^O$ denote the set of all adjacent pairs. Substituting $\adjacent_\pset^O$ for $\adjacent^O$ can directly extend \Cref{thm:computational}.}.

% Say $\omega=(a,b),\omega^\prime=(a^\prime,b^\prime)$ adjacent if $|a-a^\prime|=1$ and $b=b^\prime$. Let $\adjacent_\pset^O$ denote the set of all adjacent pairs $(\omega,\omega^\prime)$ here.

Then the program can be written as
\begin{align}\label{program-oblivious}
&\max_{\pi} \quad \sum_{\omega\in \Omega}\sum_{a} \pi(a|\omega)\mu(\omega)v(a,\omega) \notag\\
& \begin{array}{r@{\quad}l@{}l@{\quad}l}
s.t.& \sum_{\omega} u(a,\omega)\pi(a|\omega)\mu(\omega)\geq \sum_{\omega} u(a^\prime,\omega)\pi(a|\omega)\mu(\omega), & \text{ for all }a,a^\prime\\
&\sum_{a}\max\{0,\pi(a| \omega)-e^\epsilon \pi(a|\omega^\prime)\}\leq \delta, &\text{ for all }(\omega,\omega^\prime)\in\adjacent^O\\
&\sum_a \pi(a|\omega)=1, & \text{ for all }\omega\\
&\pi(a|\omega)\geq 0, & \text{ for all }a,\omega
\end{array} .
\end{align}

% The program can then be written as:
% \begin{align}
% &\max_{\pi} \quad \sum_{\omega\in \Omega}\sum_{a} \pi(a|\omega)\mu(\omega)v(a,\omega) \notag\\
% & \begin{array}{r@{\quad}l@{}l@{\quad}l}
% s.t.& \sum_{\omega} u(a,\omega)\pi(a|\omega)\mu(\omega)\geq \sum_{\omega} u(a^\prime,\omega)\pi(a|\omega)\mu(\omega), & \text{ for all }a,a^\prime\\
% &\sum_{a}\max\{0,\pi(a| \omega)-e^\epsilon \pi(a|\omega+1)\}\leq \delta, &\text{ for all }\omega\in\{0,1,\cdots,n-1\}\\
% &\sum_{a}\max\{0,\pi(a| \omega+1)-e^\epsilon \pi(a|\omega)\}\leq \delta, &\text{ for all }\omega\in\{0,1,\cdots,n-1\}\\
% &\sum_a \pi(a|\omega)=1, & \text{ for all }\omega\\
% &\pi(a|\omega)\geq 0, & \text{ for all }a,\omega
% \end{array} .
% \end{align}

For \privacyone, the privacy constraints can be written as
% \begin{align*}
% &\pi(a|\omega)\leq e^\epsilon \pi(a|\omega+1), & \text{ for all }a\text{ and }\omega\in\{0,1,\cdots,n-1\}\\
% &\pi(a|\omega+1)\leq e^\epsilon \pi(a|\omega), & \text{ for all }a\text{ and }\omega\in\{0,1,\cdots,n-1\}.\\
% \end{align*}
\[
\pi(a|\omega)\leq e^\epsilon \pi(a|\omega^\prime), \text{ for all }a\text{ and }(\omega,\omega^\prime)\in\adjacent^O.
\]

% For \privacytwo, the program requires the additional constraint:
% \[
% \sum_{s\in S}\max\{0,\pi(s| \omega)-e^\epsilon \pi(s|\omega^\prime)\}\leq \delta, \text{ for all }\omega,\omega^\prime \text{ adjacent}.
% \]


% For \privacythree, privacy constraints should be 
% \[
% \sum_{a}\pi(a|\omega)\left(\frac{\pi(a|\omega)}{\pi(a|\omega^\prime)}\right)^{\alpha-1}\leq e^{(\alpha-1)\epsilon}, \text{ for all }(\omega,\omega^\prime)\in\adjacent^O.
% \]

Program \eqref{program-distribution2} and Program \eqref{program-oblivious} are equivalent under all the above privacy constraints. Missing proofs in this section can be found in \Cref{proof_sec_computational}.
Note that only polynomial variants and constraints are in Program \eqref{program-oblivious}. We then obtain that it is a polynomial-size convex program, which implies an efficient algorithm.

\begin{lemma}\label{thm:computational}
    Under \Cref{prior-assump} and \Cref{utility-assump}, there exists an oblivious privacy-preserving signaling scheme that is optimal among all privacy-preserving signaling schemes, which means the oblivious method without loss. Therefore, there exists a polynomial-time algorithm to find the optimal signaling scheme.
\end{lemma}
\shuran{We probably do not want to make this result a main theorem. If I remember correctly, the previous paper had a similar result. It should be a lemma and the details could be moved to the appendix. }
\yuqi{change it to lemma now. The proof details are already in the appendix, while the introduction of notations and assumptions may be more appropriate to be put here?} \hf{If nonthing significant in this subsection, we should switch its order with the next section, to downgrade it.}
\yuqi{change the model into multiple receivers here}


% \begin{fact}
%     The program under \privacythree is a convex program.
% \end{fact}

% \begin{corollary}\label{coro:polynomial}
%     There exists a polynomial algorithm to find the optimal signaling scheme.
% \end{corollary}


    





==> archive/partial.tex <==
\subsection{Partial Privacy}
In real-world examples, sometimes the sender doesn't need to protect differential privacy for all adjacent pairs. We present two possible situations here.
\begin{example}
    When people use some apps, they have the opportunity to choose whether or not to consent to the disclosure of their information. Therefore, for the advertising example, sometimes the sender doesn't need to protect every web user's privacy.
\end{example}
\begin{example}
    The state sometimes contains more things than users' data. In the advertising example, the state can be two parts: the first part is whether users are the targeted customers for the advertisers, and the second part is inherent attributes of the ad space, such as size, location, stability, average number of views, etc. The seller only needs to protect the first part's differential privacy.
\end{example}

We define a set $S$ to denote all bits in the state whose privacy needs to be protected. Then the definition of adjacent pairs needs corresponding modification. Specifically, we say $\theta,\theta^\prime$ adjacent if and only if they have only one different bit and this bit is in $S$, that is $(\theta,\theta^\prime)\in \adjacent_S\Leftrightarrow\exists i\in S, \theta_i\neq \theta^\prime_i,\theta_{-i}=\theta^{\prime}_{-i}$.
$\adjacent_S$ is the set of all adjacent pairs here.

The program in the form of posterior can be written as 
\begin{align}\label{program-posterior-partial}
&\max_{\tau} \mathbb{E}_{q_s\sim \tau}[\varv(q_s)] \notag\\
& \begin{array}{r@{\quad}l@{}l@{\quad}l}
s.t.& \mathbb{E}_{q_s\sim \tau}[q_s(\theta)]=\mu_0(\theta), \text{ for all }\theta,\\
&\mathbb{E}_{q_s\sim \tau}\left[\max\left\{0,\left(\frac{q_s(\theta)}{\mu_0(\theta)}-e^\epsilon\frac{q_s(\theta^\prime)}{\mu_0(\theta^\prime)}\right)\right\}\right]\leq \delta,  \text{ for all }(\theta,\theta^\prime)\in\adjacent_S.
\end{array} .
\end{align}

Since the only difference between \Cref{program-posterior} and \Cref{program-posterior-partial} is the number of privacy constraints, We can directly extend the result in \Cref{sec-general-characterization}. 

For \privacyone, the feasible region $K(\mu_0,\epsilon)$ is $\{q\in\Delta(\Theta):q(\theta)\mu_0(\theta^\prime)/(q(\theta^\prime)\mu_0(\theta))\leq e^\epsilon\text{ for all }(\theta,\theta^\prime)\in \adjacent_S\}$.

\begin{proposition}
    The maximized utility of the sender under \privacyone is $\hullvarv(\mu_0\mid K(\mu_0,\epsilon))$. Also, the optimal signal scheme is inducing posteriors in $S_{\varv}(\mu_0\mid K(\mu_0,\epsilon))$ with $|S_{\varv}(\mu_0\mid K(\mu_0,\epsilon))|$ signals.
\end{proposition}

For \privacytwo,
the modified function $\varvtwo: \Delta(\Theta)\times\mathbb{R}^{|\adjacent_S|}\mapsto \mathbb{R}$ is
\[
    \varvtwo(q,\gamma)=\varv(q).
\]
The feasible region is
\[
C(\mu_0,\epsilon):=\left\{(q,\gamma)\in \Delta(\Theta)\times \mathbb{R}^{|\adjacent_S|}:\max\left\{0,\left(\frac{q(\theta)}{\mu_0(\theta)}-e^\epsilon\frac{q(\theta^{\prime})}{\mu_0(\theta^{\prime})}\right)\right\}\leq \gamma_{\theta,\theta^\prime}, \text{ any }(\theta,\theta^\prime)\in \adjacent_S\right\}.
\]
\begin{proposition}
The maximized utility of the sender under \privacytwo for $S$ is $\hullvarvtwo(\mu_0,\bm{\delta}\mid C(\mu_0,\epsilon))$, where $\bm{\delta}$ is the $|\adjacent_S|$-dimension vector with all elements $\delta$. Also, the optimal signal is inducing posteriors in $S_{\varvtwo}(\mu_0,\bm{\delta}\mid C(\mu_0,\epsilon))$ with $|S_{\varvtwo}(\mu_0,\bm{\delta}\mid C(\mu_0,\epsilon))|$ signals.
\end{proposition}

For computational results, we first modify the projection $\phi$:
\[
\phi_S(\theta)\coloneqq (\sum_{i\in S}\theta_i,\sum_{i\notin S}\theta_i).
\]
We also update the meaning of adjacent. Say $\omega=(a,b),\omega^\prime=(a^\prime,b^\prime)$ adjacent if $|a-a^\prime|=1$ and $b=b^\prime$.
Then the program \ref{program-oblivious} can be written as
\begin{align*}
&\max_{\pi} \quad \sum_{\omega\in \Omega}\sum_{a} \pi(a|\omega)\mu_0(\omega)v(a,\omega) \notag\\
& \begin{array}{r@{\quad}l@{}l@{\quad}l}
s.t.& \sum_{\omega} u(a,\omega)\pi(a|\omega)\mu_0(\omega)\geq \sum_{\omega} u(a^\prime,\omega)\pi(a|\omega)\mu_0(\omega), & \text{ for all }a,a^\prime\\
&\sum_{a}\max\{0,\pi(a| \omega)-e^\epsilon \pi(a|\omega^\prime)\}\leq \delta, &\text{ for all }\omega,\omega^\prime \text{ adjacent}\\
&\sum_a \pi(a|\omega)=1, & \text{ for all }\omega\\
&\pi(a|\omega)\geq 0, & \text{ for all }a,\omega
\end{array} .
\end{align*}
Then similar results can be obtained as \Cref{sec-computational}.
\begin{assumption}\label{prior-assump-partial}
    If $\phi_S(\theta)=\phi_S(\theta^\prime)$, then $\mu_0(\theta)=\mu_0(\theta^\prime)$.
\end{assumption}
\begin{assumption}\label{utility-assump-paritial}
    If $\phi_S(\theta)=\phi_S(\theta^\prime)$, then $u(a,\theta)=v(a,\theta^\prime)$ and $v(a,\theta)=v(a,\theta^\prime)$ for any $a$.
\end{assumption}

\begin{proposition}
    Under \Cref{prior-assump-partial} and \Cref{utility-assump-paritial}, there exists an oblivious privacy-preserving signal scheme that is optimal among all privacy-preserving signal schemes, which implies the oblivious method is without loss. Also, there exists a polynomial algorithm to find the optimal signal scheme.
\end{proposition}




==> archive/renyi.tex <==
\subsection{Other privacy constraints}
\yuqi{needs reorganized}
\begin{definition}
     A data publication mechanism $(S, \pi)$ is $(\alpha,\epsilon)$-Rényi differentially private if for all databases $\theta, \theta^{\prime} \in \Theta$ that are adjacent, in the sense that they differ in at most one entry (i.e., such that for some $\left.n \in\{1, \ldots, N\}, \theta_{-n}=\theta_{-n}^{\prime}\right)$, we have 
$$
\mathrm{D}_\alpha\left(\pi(\cdot|\theta) \| \pi(\cdot|\theta^\prime)\right) \leq\epsilon,
$$
where $\mathrm{D}_\alpha(\pi(\cdot|\theta) \| \pi(\cdot|\theta^\prime))$ is the $\alpha $-Rényi divergence between the two distributions $\pi(\cdot|\theta)$ and $\pi(\cdot|\theta^\prime)$.
\end{definition}

\begin{definition}
    Let $P$ and $Q$ be probability distributions on $\Omega$. For $\alpha \in(1, \infty)$, we define the Rényi divergence of order $\alpha$ between $P$ and $Q$ as
$$
\begin{aligned}
\mathrm{D}_\alpha(P \| Q) & =\frac{1}{\alpha-1} \log \left(\int_{\Omega} P(x)^\alpha Q(x)^{1-\alpha} \mathrm{d} x\right) \\
& =\frac{1}{\alpha-1} \log \left(\underset{x \sim Q}{\mathbb{E}}\left[\left(\frac{P(x)}{Q(x)}\right)^\alpha\right]\right) \\
& =\frac{1}{\alpha-1} \log \left(\underset{x \sim P}{\mathbb{E}}\left[\left(\frac{P(x)}{Q(x)}\right)^{\alpha-1}\right]\right),
\end{aligned}
$$
where $P(\cdot)$ and $Q(\cdot)$ are the probability mass/density functions of $P$ and $Q$.
\end{definition}

For $(\alpha,\epsilon)$-zero-concentrated differential privacy, the program requires the additional constraint:
\[
\sum_{s\in S}\pi(s|\theta)\left(\frac{\pi(s|\theta)}{\pi(s|\theta^\prime)}\right)^{\alpha-1}\leq e^{(\alpha-1)\epsilon}, \text{ for all }\theta,\theta^\prime \text{ adjacent}.
\]


$(\alpha,\epsilon)$-zero-concentrated differential privacy can be written as
\[
\mathbb{E}_{q_s\sim \tau}\left[\left(\frac{q_s(\theta)}{\mu_0(\theta)}\right)^{\alpha}\left(\frac{q_s(\theta^\prime)}{\mu_0(\theta^\prime)}\right)^{1-\alpha}\right]\leq e^{(\alpha-1)\epsilon},  \text{ for all }\theta,\theta^\prime \text{ adjacent}.
\]


\begin{proposition}\label{biprivacythree}
    We define $t_1=q_{s_1}(1-\mu_0)/((1-q_{s_1})\mu_0)$ and $t_2=q_{s_2}(1-\mu_0)/((1-q_{s_2})\mu_0)$. We also define a distribution $\sigma$ with binary support on $\{t_1,t_2\}$. Also, $\sigma(t_1)=\frac{1-q_{s_1}}{1-\mu_0}\tau(q_{s_1})$ and $\sigma(t_2)=\frac{1-q_{s_2}}{1-\mu_0}\tau(q_{s_2})$. The signal scheme preserves \privacythree if and only distribution $\sigma$ satisfy:
    \[
    \begin{cases}
        \mathbb{E}_\sigma[t]=1\\
        \mathbb{E}_\sigma[t^\alpha]\leq e^{(\alpha-1)\epsilon}\\
        \mathbb{E}_\sigma[t^{1-\alpha}]\leq e^{(\alpha-1)\epsilon}.
    \end{cases}
    \]
\end{proposition}
\begin{proof}
    Recall the \privacythree constraint in the program using the form of posteriors:
    \[
    \mathbb{E}_{q_s\sim \tau}\left[\left(\frac{q_s(\theta)}{\mu_0(\theta)}\right)^{\alpha}\left(\frac{q_s(\theta^\prime)}{\mu_0(\theta^\prime)}\right)^{1-\alpha}\right]\leq e^{(\alpha-1)\epsilon},  \text{ for all }\theta,\theta^\prime \text{ adjacent}.
    \]
    % Since $q_{s_2}\geq q_{s_1}$ and $\mathbb{E}[q_s]=\mu_0$, we have $q_{s_2}\geq \mu_0\geq q_{s_1}$. Also, $\tau(q_{s_1})=(q_{s_2}-\mu_0)/(q_{s_2}-q_{s_1})$ and $\tau(q_{s_2})=(\mu_0-q_{s_1})/(q_{s_2}-q_{s_1})$.
    Then we obtain
    \begin{align*}
        &\left(\frac{q_{s_1}}{\mu_0}\right)^\alpha\left(\frac{1-\mu_0}{1-q_{s_1}}\right)^{\alpha-1}\tau(q_{s_1})+\left(\frac{q_{s_2}}{\mu_0}\right)^\alpha\left(\frac{1-\mu_0}{1-q_{s_2}}\right)^{\alpha-1}\tau(q_{s_2})\leq e^{(\alpha-1)\epsilon},\\
        &\left(\frac{1-q_{s_1}}{1-\mu_0}\right)^\alpha\left(\frac{\mu_0}{q_{s_1}}\right)^{\alpha-1}\tau(q_{s_1})+\left(\frac{1-q_{s_2}}{1-\mu_0}\right)^\alpha\left(\frac{\mu_0}{q_{s_2}}\right)^{\alpha-1}\tau(q_{s_2})\leq e^{(\alpha-1)\epsilon}.
    \end{align*}
    We then define $t_1,t_2,\sigma(t_1),\sigma(t_2)$ as the theorem. Substituting them into the above equations, we have
    \begin{align*}
        &t_1^{\alpha}\sigma(t_1)+t_2^\alpha\sigma(t_2)\leq e^{(\alpha-1)\epsilon},\\
        &t_1^{1-\alpha}\sigma(t_1)+t_2^{1-\alpha}\sigma(t_2)\leq e^{(\alpha-1)\epsilon}.
    \end{align*}
    Also, $t_1\sigma(t_1)+t_2\sigma(t_2)=(q_{s_1}\tau(q_{s_1})+q_{s_2}\tau(q_{s_2}))/\mu_0=1$.
\end{proof}

Under \privacythree, the program is
\begin{align*}
&\max_{\tau} \mathbb{E}_{q_s\sim \tau}[\varv(q_s)] \\
& \begin{array}{r@{\quad}l@{}l@{\quad}l}
s.t.& \mathbb{E}_{q_s\sim \tau}[q_s(\theta)]=\mu_0(\theta), \text{ for all }\theta,\\
&\mathbb{E}_{q_s\sim \tau}\left[\left(\frac{q_s(\theta)}{\mu_0(\theta)}\right)^{\alpha}\left(\frac{q_s(\theta^\prime)}{\mu_0(\theta^\prime)}\right)^{1-\alpha}\right]\leq e^{(\alpha-1)\epsilon},  \text{ for all }\theta,\theta^\prime \text{ adjacent}.
\end{array} .
\end{align*}


\paragraph{A modified objective function for \privacythree}
Similarly, for \privacythree, we use the modified function $\varvtwo$ and define
\[
C^\prime(\mu_0,\alpha):=\left\{(q,\gamma)\in \Delta(\Theta)\times \mathbb{R}^{m}:\left(\frac{q(\theta)}{\mu_0(\theta)}\right)^{\alpha}\left(\frac{q(\theta^{\prime})}{\mu_0(\theta^{\prime})}\right)^{1-\alpha}\leq \gamma_{\theta,\theta^\prime}, \text{ any }(\theta,\theta^\prime)\text{ adjacent}\right\}.
\]
% Then we modify the function $\varv$ to $\varv^{2}_{\mu_0,\alpha}: \Delta(\Theta)\times \mathbb{R}^{m}\mapsto \mathbb{R} \cup\{ \pm \infty\}$ as 
% \[
% \varv^{2}_{\mu_0,\alpha}(q,\gamma)=\varv(q)-\delta(q,\gamma|C^\prime(\mu_0,\alpha)),
% \]

%  we also modify the definition of concave hull in \ref{eq:concavehull} slightly:
% \begin{align*}
%  \varv^+(x,y) &\coloneqq \max_{T\subseteq \Delta(\Theta)\times\mathbb{R}^m, |T|\leq k+m}\Biggl(\sum_{(x_i,y_i)\in T}\tau((x_i,y_i))\varv(x_i,y_i): \sum_{(x_i,y_i)\in T}\tau((x_i,y_i))x_i=x,\\
%  &\qquad \sum_{(x_i,y_i)\in T}\tau((x_i,y_i))y_i=y, \sum_{(x_i,y_i)\in T}\tau((x_i,y_i))=1, \tau((x_i,y_i))\geq 0\Biggr).
% \end{align*}
% \yuqi{use the same concave hull definition, area, Q}


We then characterize the problem with the concave hull of $\varvtwo$.

\begin{proposition}
The maximized utility of the sender under \privacythree is $\hullvarvtwo(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))$, where $\bm{e^{(\alpha-1)\epsilon}}$ is the $m$-dimension vector with all elements $e^{(\alpha-1)\epsilon}$. Also, the optimal signal scheme is inducing posteriors in $S_{\varvtwo}(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))$ with $|S_{\varvtwo}(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))|$ signals.
\end{proposition}

\begin{corollary}\label{bene-pri-three}
    Sender benefits from persuasion under \privacythree if and only if $\hullvarvtwo(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))>\varv(\mu_0)$.
\end{corollary}
\begin{proposition}
    Under \privacythree, if $\varvtwo$ is concave in $C^\prime(\mu_0,\alpha)$, the sender does not benefit from persuasion for any prior. If $\varvtwo$ is convex and not concave in $C^\prime(\mu_0,\alpha)$, the sender benefits from persuasion for any prior.
\end{proposition}

Say \benefit under \privacythree if there exists $(q,\gamma)\in C^\prime(\mu_0,\alpha)$ that
\[
\varvtwo(q,\gamma)=\varv(q)>\E_{\theta\sim q}[ v\left(\hat{a}\left(\mu_0\right), \theta\right)].
\]



Similarly, for \privacythree, we use the modified function $\varvtwo$ and define
\[
C^\prime(\mu_0,\alpha):=\left\{(q,\gamma)\in \Delta(\Theta)\times \mathbb{R}^{|A_S|}:\left(\frac{q(\theta)}{\mu_0(\theta)}\right)^{\alpha}\left(\frac{q(\theta^{\prime})}{\mu_0(\theta^{\prime})}\right)^{1-\alpha}\leq \gamma_{\theta,\theta^\prime}, \text{ any }(\theta,\theta^\prime)\in A_S\right\}.
\]
\begin{proposition}
The maximized utility of the sender under \privacythree is $\hullvarvtwo(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))$, where $\bm{e^{(\alpha-1)\epsilon}}$ is the $|A_S|$-dimension vector with all elements $e^{(\alpha-1)\epsilon}$. Also, the optimal signal scheme is inducing posteriors in $S_{\varvtwo}(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))$ with $|S_{\varvtwo}(\mu_0,\bm{e^{(\alpha-1)\epsilon}}\mid C^\prime(\mu_0,\alpha))|$ signals.
\end{proposition}

